VizRec: A framework for secure data exploration via visual representation

Visual representations of data (visualizations) are tools of great importance and widespread use in data analytics as they provide users visual insight to patterns in the observed data in a simple and effective way. However, since visualizations tools are applied to sample data, there is a a risk of visualizing random fluctuations in the sample rather than a true pattern in the data. This problem is even more significant when visualization is used to identify interesting patterns among many possible possibilities, or to identify an interesting deviation in a pair of observations among many possible pairs, as commonly done in visual recommendation systems. We present VizRec, a framework for improving the performance of visual recommendation systems by quantifying the statistical significance of recommended visualizations. The proposed methodology allows to control the probability of misleading visual recommendations using both classical statistical testing procedures and a novel application of the Vapnik Chervonenkis (VC) dimension method which is a fundamental concept in statistical learning theory.

==> experiments.tex <==
\section{Experimental evaluation}\label{sec:experiments}
% \begin{itemize}
%     \item non-viz would lead to noise (i.e. contrast with SeeDB)
%     \begin{itemize}
%         \item can show example of Multicomparison problem (a notebook for this exists somewhere)
%         \item Further, can do example bar with very close distributions across many bars. VC won't pick up, but chi2 would. (though we have this already in the constructed example).
%     \end{itemize}
%     \item Constructed example: We have an example where chi2 recommends it, however the epsilon distance is not significant enough for visualization purposes. VC would not pick it up.
%     \item limited number of queries and $\chi^2$
%     \begin{itemize}
%         \item Show plot chi2 distance vs. minimum number of samples required to perform it. (cf. \autoref{fig:chi2minsamples}) 
%         \item Conclusion: For chi2 estimating observed probabilities is more critical than the actual distance metric. I.e. if we guarantee good estimates for observed (and expected) probabilities, then if there is a min-distance between these two, Chi2 will also correctly select this. Even at very high number of hypothesis.
        
%         \item If we do not have enough samples, then Fisher's exact test should be performed
%     \end{itemize}
%     \item How selective something needs to be? (cf. \autoref{fig:selectivity})
%     \begin{itemize}
%         \item show experiment VC dimension selectivity for different dimensions (exclude Chi2 due to previous explanation) \leo{perform experiment with inverse search to stabilize results?}
%     \end{itemize}
%     \item anecdotal example
%     \item AirBnB anecdotal examples? Can i.e. use distributions over shared apartment number of bathrooms/bedrooms, ...
%     \item ranking under different distances (KL, EMD, chi2 dist, Minkowski, ...): Use a Bin(n, 0.5) as reference. Then, use Bin(n, p) with p varied over 0.5-1.0 as query. What biases (p) would techniques select under different ranking measures? table of top5. Also idea could be to do min/max bias/measure of each selected measure under this setup.
%     \item rare bars/missing bar case: Chi2 requires rule of thumb at least 5 observations in each bin. This is not practical. What to do? Pseudocounts? ignpre testing? etc. maybe can even find an anecdotal example of this. VC dim has no problem with it.
% \end{itemize}

\tim{(1) Anecdotal showing top-3 SeeDB recommendations vs controlled. Ideally not the top-1 form SeeDB is the same as controlled}

\tim{(2) Use Anecdotal survey to show that without a clever restriction of the search space nothing (or little) gets recommended. With the proposed heuristic, we get recommendations. }

\tim{(3) Visualize that every interaction of the user can indicate if the visualization is safe using VC dimensions only (again anecdotal case)  }

\tim{(4) Bonferroni vs VC Dimensions vs Chernoff bounds - what type of visualization with visual significance are recommendet -   figs/chi2vsvc_example.png . If possible find anecdotal}

\tim{(5) Show the power of VC Dim. vs Chernoff - Figure 6}

In this section we want to demonstrate some of the challenges that developers face when designing a statistically safe visual recommendation system like VizRec. Though at first sight the two proposed techniques based on classical statistical testing or statistical learning seem to be directly comparable, we show in this section that they do in fact provide different guarantees, are not interchangeable and need to be chosen thus depending on both the given scenario and the desired statistical guarantee. I.e. if a user only wants guarantee he may use statistical tests, if instead he always wants to guarantee a meaningful statistical difference we advice to use either statistical tests with appropriate hypothesis our the statistical learning approach presented in \autoref{sec:vcapproach}.
\subsection{Exp1: Random data should not lead to any recommendations}
In our first experiment, we want to show that it is essential to employ statistical guarantees when building visual recommender systems. To demonstrate that both techniques will not recommend false positives, we generated a synthetic dataset with uniformly distributed data. $100,000$ samples were generated in total with the first column being selected as aggregate and the other 3 columns as features. The aggregate is uniformly distributed over $\lbrace 1, 2, 3, 4\rbrace$ and each of the $3$ features uniformly distributed over the set $\lbrace 1, ..., 9 \rbrace$.
\begin{figure}[ht!]
\centering
     \includegraphics[width=\columnwidth]{figs/pvals_uniform.png}
\caption{P-values displayed were sorted after their value. Most of them are larger than the chosen significance level of $\alpha=0.05$. However, when running multiple $\chi^2$-tests under the same significance level inevitably the multiple comparisons problem will manifest itself as demonstrated here. By chance, though there is no evidence in the data, p-values smaller than $\alpha$ occur. Adding a FWER will avoid these problem but may lead to overly conservative significance levels to test for.}
\label{fig:exp1_pvals}
\end{figure}
With simple predicates (i.e. a queries formed from $\leq$ clauses solely) there were 1331 visualizations to be explored (a dummy value of $+\infty$ was used in the queries to make a feature active or not. E.g. consider a query of the form $\left( X_1 \leq 8 \right) \land \left( X_2 \leq +\infty \right) \land \left( X_3 \leq 3 \right)$. In this query, feature $X_2$ has no effect on the rows returned since $\left( X_1 \leq 8 \right) \land \left( X_2 \leq +\infty \right) \land \left( X_3 \leq 3 \right) \equiv \left( X_1 \leq 8 \right) \land \left( X_3 \leq 3 \right)$. Note that using $+\infty$-values in the clauses does not change the VC dimension.). As a reference, a uniform distribution over $\lbrace 1, 2, 3, 4\rbrace$ was chosen, i.e. $\mathbb{P}(X = k) = 1/4$ for $k=1, ..., 4$. This means, that the expected support of any visualization is at least $10^5/9^3$ samples which is a fair amount to estimate $4$ bars. A VRS effectively using statistical guarantees should not pick up any visualization since there is no difference within the data.
\begin{figure}[ht!]
\centering
    %  \includegraphics[width=\columnwidth]{figs/vc_uniform.png}
    \includegraphics[width=\columnwidth]{figs/vc_uniform_NEW.png}
\caption{Interest scores based on the suggested Chebyshev-metric were computed for all visualizations. $\epsilon$ guarantees the bound at $\delta = 0.05$, however it needs to be corrected for the selectivity each visualization is based on. Else, wrong (random) visualizations would get recommended. As seen in this graph, the VC dimension approach effectively controls that no visualization gets recommended from random, noisy data. The VC-dimension of the class all queries belong to reflects the shape of the $\overline{\epsilon}$ curve shown here. I.e. the lower the dimension the more the shape takes the form of an L. Here, a dimension of $4$ is shown.}
\label{fig:exp1_vc}
\end{figure}
\\\\
When not accounting for the multiple comparison problem p-values below the threshold of $\alpha=0.05$ occur, as depicted in \autoref{fig:exp1_pvals}, inevitably. A system without FWER or FDR guarantees would classify them as false positives. Using Bonferroni (or other comparable corrections) remedies this as demonstrated in \autoref{fig:exp1_pvals}.
\\
\\
In comparison the lowest $\epsilon$ the VC approach guarantees is $\epsilon_{\min} = 0.0059$. As discussed in \ref{ConcreteVC} the required threshold $\overline{\epsilon}$ to be met by the Chebychev norm induced distance measure $d_\infty$ depends on the selectivity $\gamma$ of the query. The necessity of such a scaling can be observed in \autoref{fig:exp1_vc} too. With the interest scores(distances) being lower for all queries in \autoref{fig:exp1_vc} the VC approach does not recommend any false positives in this experiment. Using different distributions instead of the uniform one showed comparable results.
\subsection{Exp2: Statistical testing guarantees only difference but not significant difference}
For our second experiment, we want to show that statistical testing in the form of a \chisqtest is in general not a wrong ingredient for building a VRS but lacks the ability to spot meaningful, visual differences and whether they are justified by the sample size. Similar results hold for the $t$-test or Kolmogorov-Smirnov test.
\\
\\
Assume we had a query that yielded $m=1,200$ out of $n=10,000$ samples and a perfect estimator for the true distribution function of the reference and the query distribution. These distributions shall be distributed as in \autoref{fig:exp2_chi2vsvc}. Thus, the \chisqtest would yield a p-value of of $2.54 \cdot 10^{-5}$ implying that they are different when not more than $1967$ visualizations under Bonferroni's correction are tested.
\begin{figure}[ht!]
\centering
     \includegraphics[width=\columnwidth]{figs/chi2vsvc_example.png}
\caption{Comparing two close distributions that however should not be recommended since the visual difference criterion according to the VC dimension approach is not met. Using $\chi^2$ test would recommend this visualization since it only spots that there is a difference but not whether the difference is significant enough.}
\label{fig:exp2_chi2vsvc}
\end{figure}
However, at a VC dimension of 10 ($\delta=0.05$) the required $\overline{\epsilon}$ must be at least $0.22$ which is nearly twice as high as the $0.1$ difference at the first bar as shown in \autoref{fig:exp2_chi2vsvc}. Thus, the VC approach would not select this visualization as being significantly different enough given the modest sample size. Similar examples yielding comparable results can be constructed to show that cases exist where the $\chi^2$ test would be pick up a visually not significantly enough signal in the data.
\\
\\
In practice, scenarios like the one presented here occur especially due to outliers in the data. I.e. it could happen that for one feature value there are only 1-5 samples that would lead without any correction to a positive recommendation. Though a heuristic may ignore visualizations with less than $5$ samples, this would come at the cost of ignoring rare phenomena and by using some magic number to define the threshold. I.e. when ignoring visualizations with less than $b$ samples per bin, easily an example with $b+1$ samples for some bin could be found where $\chi^2$ would pick up a non-visually significant visualization.
\\
\\
This underscores that a VRS using the \chisqtest would correctly identify two visualizations being different but can not guarantee a meaningful difference in terms of a distance which is crucial to build usable systems without luring the user into a false sense of security. One may argue that filtering out visualizations after having performed statistical testing would remedy this(which may work in practice when the interest score is high enough), but then there was no guarantee that the distances observed is statistically guaranteed.
\\
\\
Whereas the question is dependent on the scenario (i.e. which query and which guarantees a system needs to fulfill) we want to point out, that there is a simple way to use the \chisqtest to control significant distance too. As described in \cite{chi2book} by modifying the \chisqtest to 
test a more complex null hypothesis
\begin{equation}
H_0: \sum_{k=1}^K \frac{\left( p_k - \hat{p}_k \right)^2}{p_k} < \epsilon_{\chi^2}
\end{equation}
together with the corresponding test statistic 
\[
T = n\gamma \sum_{k=1}^K \frac{\left( p_k - \hat{p}_k \right)^2}{p_k}
\]
following a non-central $\chi^2$ distribution with $K-1$ degrees of freedom and non-locality parameter 
\[
\lambda_{\mathrm{nc}} = n \gamma \epsilon_{\chi^2} = m \epsilon_{\chi^2}.
\]
The distance guaranteed then is the $\chi^2$-distance $d_{\chi^2}$. In fact, this testing procedure can be further generalized to use other distances that belong to the family of f-divergences like the total variation distance or Kullback-Leibler divergence via an suitable transformation or by using non-parametric models to estimate the distance measures before comparing them via statistical testing as in described in more detail in \cite{fdivergence}.
\leo{m = how many samples query yielded, n total number of samples}
% \leo{todo: mention here Chi2 with more general null hypothesis as in }
\subsection{Exp3: Accurate estimation of relative frequency is crucial}
In this experiment we want to show that the Chi-squared test is indeed a very powerful test but that the correct estimation of the distribution dominates the selectivity or in other words the number of samples a query yields. In other words, when we guarantee that the estimates for the probability mass function are close enough to the true values a testing procedure like \chisqtest will even under a million possible hypothesis only need a small number of samples to spot a difference between two distributions. We thereby define the required number of point estimates to be in the range of $K=2, .., 100$ bars as meaningful for visualization recommender systems (cf. \autoref{fig:exp3_minchi2}).
\begin{figure}[ht!]
\centering
     \includegraphics[width=\columnwidth]{figs/minsampleschi2.png}
\caption{Chi-square distance $d_{\chi^2}$ and minimum number of samples $n_{\mathrm{min}}$ required for the \chisqtest to reject the null hypothesis assuming Bonferroni correction with $\alpha' = 0.05$ and $10^6$ queries.}
\label{fig:exp3_minchi2}
\end{figure}
In \autoref{fig:exp3_minchi2} it is shown that even low values for the $\chi^2$-distance $d_\chi^2$ only require queries with hundreds of samples to be identified correctly.
\subsection{Exp4: Single Visualization vs. Multiple Visualization setting}
In this experiment, we want to show that when only a single visualization needs to be recommended, using Chernoff-Hoeffding bounds is both easier and yields a better guarantee than a VC-based bound. However, when testing multiple visualizations on the same data, the VC approach dominates Chernoff-Hoeffding bounds.
\begin{figure}[ht!]
\centering
     \includegraphics[width=\columnwidth]{figs/chernoffvsvc.png}
\caption{Observed estimation error for a single random experiment and bounds obtainable at a significance level of $\delta = 0.05$. For a VC dimension of $d=1$, the bound is only slightly worse than the Chernoff bound of a single visualization. However, with increasing number of visualizations Chernoff bounds are more conservative than bound obtained via VC.}
\label{fig:exp4_chernoffvsvc}
\end{figure}
To show this, random data was generated to estimate the probability mass function of a biased Binomial distributed according to $\sim \mathrm{Bin}(10, 0.3)$. In \autoref{fig:exp4_chernoffvsvc} a sample path is shown together with the theoretical bounds for a setup with a VC dimension of $2$. Comparing to a Chernoff-Hoeffding bound of a single visualization, the VC approach outperforms Chernoff-Hoeffding bounds when learning multiple visualizations at once.
% \todo{I feel the Chernoff thing should be included in the theory section}
% \todo{Can also produce a plot to show how many visualizations are required to outperform Chernoff for 5 bars, 10bars, ...}

% \subsection{Exp5: Real-world data}
% In this experiment we want show an actual example on how to apply the VC approach to real data. Therefore, we scraped AirBnB for pricing data around Boston resulting in a small to medium sized data sets of $6125$ rows after cleaning. In particular we are interested in exploring the distribution of prices and how they are connected to the ordinal attributes \#bedrooms, \#bathrooms and the categorical attributes zipcode, roomtype and city. Prices have been binned into 6 bings ranging from \$0 to \$500. When using queries that combine multiple $=$ clauses, the vc dimension is here $15$ (since we also want to exclude attributes) which results in an $\epsilon = 0.038$ at $\delta=0.05$. Without any preprocessing, the significance level to test for originating from $\alpha'=0.05$ when applying Bonferroni correction is a very low $\alpha = 6 \cdot 10^{-8}$ for 

==> fwer.tex <==

%\section{FWER control using VC dimension}
% While the control through $\chi^2$ can prove effective in many scenarios, it also presents several drawbacks.
% \begin{itemize}
%     \item \textbf{Loss of statistical power:} the statistical power of classical testing procedures noticeably decrease as the number of hypotheses being tested increases. This is an effect of the fact that most multiple hypotheses correction techniques (e.g., Bonferroni, Holm, Hoechemberg) operate by strengthening the threshold which  is required to deem a phenomenon are statistically relevant. As the number of hypotheses gets higher and higher is becomes harder and harder to acknowledge actually statistically relevant phenomenon. While the number of false positives remains controlled, the number of false negatives will increase.
%     While some multiple hypotheses correction techniques (e.g., the Holm or the Hoechember procedures) allows consistent improvements over the simpler Bonferroni procedure, they are still affected by this phenomenon, especially in setting for which the number of true positives is low.
%     In the extreme case, when the number of possible filters, and hence visualizations, to be considered in infinite any FWER multiple hypothesis correction loses its applicability as the only hypotheses that are rejected are those for which the $p$-value equal zero.
%     \item \textbf{Scalability:} 
%     When applying this classical FWER controlling techniques it necessary to evaluate the total number of hypotheses being tested. Further it is necessary to evaluate the $p$-values of \emph{all} the hypotheses being considered.
%     \item \textbf{Edge cases:} When applying the $\chi^2$ procedure there are edge situations which have to be recognized and opportunely treated. As an example, when evaluating a visualization with $k$ buckets using the $\chi^2$ test, it is required that a minimum number of records are observed for each of these bins. While it is indeed possible to correct for this issue (i.e., by switching to Fischer's exact test) such corrections require ad-hoc on-the-fly adjustments. 
% \end{itemize}


==> strategies.tex <==
Recent work \cite{controlfd} specifically investigated how the search space of potential visualizations can be explored interactively in a ``\emph{safe  way}, that is while maintaining control of the ``\emph{Marginal False Discovery Rate}'' (mFDR). Though control via FWER techniques rules out an interactive exploration setting and also the VC method does not allow per se to explore data interactively, it can be leveraged using heuristics and preprocessing to lower the certainty required and provide more exploratory power thus. Furthermore, the VC approach provides a simple stopping criterion when exploring the search space of possibly recommendable visualizations.
\subsection{Preprocessing}
Although it is statistically wrong to apply correction mechanisms after some sort of pre-filtering or outliers removal steps in general, for real datasets certain preprocessing steps do not necessarily sacrifice statistical guarantees, even are sometimes necessary and eventually help to decrease noise in the signal in a way that discovering interesting visualizations is less sensible to random noise present in a dataset. In this section we outline several preprocessing steps which allow to impove the effectiveness of our control procedures without interfering  with the statistical guarantees provided or follow axiomatic justifications like Tarone's exclusion principle\cite{tarone}.
\begin{itemize}
    \item \textbf{Constant columns} can be safely ignored (i.e. a column where there is only one distinct value present). This will both prune the search space and reduce the necessary VC-dimension by the number of ignored columns at least.
    \item \textbf{Columns with a bad ratio of number of unique values to total number of samples} can be also removed. I.e. an ID column is useless for visualization purposes, the same goes for foreign key columns. They should be ignored whenever knowledge about their purpose is available. However, this can be also generalized to other, meaningful columns: I.e. if the number of unique features $n_{\mathrm{unique}}$ compared to the number of total samples $n$ has a ratio that makes it very likely that bins will not have many samples according to the pigeonhole principle, e.g. $n / n_{\mathrm{unique}} < 5$, the column can be ignored. This both prunes the test space and also does reduce the VC-dimension.
    \item \textbf{Highly correlated columns} may be merged. If correlations of columns are close to being a maximum (i.e. $1 - \rho^2 < \epsilon_\rho$ for a small enough $\epsilon_\rho$. Note that we want to weigh $\rho$ in a power based way) then one of the two columns may be dropped. An example of this could be redundant data, e.g. a salary that is given in different currencies.
%    \item \textbf{Binning columns} with more than e.g. $100$ unique values. After having removed id/foreign key columns, columns that have too many features should be binned. Then, other preprocessing steps (in the form of a fix point iteration) may be applied. \leo{I am not so sure about this honestly.}
    \item \textbf{Empty visualizations} may be excluded according to Tarone's exclusion principle \cite{tarone} which says that in a multiple testing setting queries with $m=0$ rows can be ignored. While there is no immediate benefit to the VC dimension, this drastically decreases the search space and allows for a better correction factor when using e.g. Bonferroni correction for Chi-square testing under family-wise error rate guarantees.
    \item \textbf{Equivalence classes} as defined in \cite{matteovc} treat queries yielding the (exact) same set of tuples as output to be a member of the same equivalence class. This may lead to fewer unique values and even exclude multiple columns from the exploration.
\end{itemize}
These preprocessing steps can be used to tune a system before recommending any visualizations. However, all tuning needs to performed before controlling for false discoveries. Else, the controls are not valid.
\subsection{Exploration Heuristic}
Finding an efficient exploration strategy remains an open problem, however depending on a system's goal greedy approaches can be used. The difficulty stems in particular from the vast nature of datasets. However, and despite often a theoretical counterexample may be constructed, we introduce in this section a heuristic that follows a practical ansatz in exploring the search space of possible recommendations.
\\
\\
Since the likelihood of having a good estimate increases with the number of observed samples, it makes sense to first test for predicates that will have good estimates. Hence, predicates should be build starting with columns having the fewest unique number of values until getting to finer grained ones. This allows to heuristically test first the likely meaningful visualizations.
\\
\\
When using $+\infty$ values additionally to deactivate/activate certain attributes, the exploration can be performed via a tree. Then, in order to prune the search space a stopping criterion can be employed. Even when not explicitly using $+\infty$-values it may be a good idea to use them and a tree based exploration when there are enough samples.
\\
\\
For statistical testing under FWER guarantees a stopping critierion may be to check for the prerequisites of a test. For example in the case of a $\chi^2$-test, whenever there are less than e.g. $5$ samples per bin, the path in the exploration tree should be no further explored. Under another guarantee, i.e. FDR, techniques like $\alpha$-investing \cite{controlfd} can be also used as stopping criterion (i.e. each branch gets assigned a certain $\alpha$-budget).
\\
The VC based approach allows for an even simpler stopping criterion. If a query does not yield enough samples to satisfy the $\epsilon/\delta$-criterion, further refining it will also violate the criterion. Thus, branches may be cut early in the exploration.
% \begin{itemize}
%     \item VC dimension: Tree with cutoff when number of samples is not sufficient.
%     \item heuristic: sort columns after number of features asc. ignore columns with a single feature (constant). Then build filters starting left to right. Why? More likely to violate VC sample requirement on high feature columns.
% \end{itemize}
% \subsubsection{Selecting which columns to use for predicate creation}
% \todo{might be also renamed to preprocessing}
% \todo{formulas for search space size? include perhaps showing how they explode?}

% Thus an exploration heuristic could look in pseudo-code like this:
% \begin{enumerate}
%     \item given total number of samples, compute highest vc-dimension $d$ that still allows epsilon/delta guarantee for given sample size.
%     \item determine number of unique features (can be done approximately)
%     \item sort asc. columns after number of unique features
%     \item remove columns with single unique feature
%     \item select up to $d - 1$ columns, depending on the type of predicates to be build (cf. \autoref{sec:relationvcpredicate}), if there are more than $d-1$ candidates, try to eliminate more of them by looking at correlations, unique feature ratios, ...
%     \item run first exploration pass, count number of empty visualizations and columns that only yielded empty visualizations
%     \item if there were $g$ columns encountered that yielded empty visualizations, add up to $g$ columns from the non-selected ones (sorted!) and run second pass refining previous visualizations further.
% \end{enumerate}
% A similar strategy can be performed when using chi-square based testing only. For Chisquare after encountering empty visualizations, the correction can be run again to determine a final set of visualizations to be recommended.
